Lower Bounds for Prior Independent Algorithms

The prior independent framework for algorithm design considers how well an algorithm that does not know the distribution of its inputs approximates the expected performance of the optimal algorithm for this distribution. This paper gives a method that is agnostic to problem setting for proving lower bounds on the prior independent approximation factor of any algorithm. The method constructs a correlated distribution over inputs that can be generated both as a distribution over i.i.d. good-for-algorithms distributions and as a distribution over i.i.d. bad-for-algorithms distributions. Prior independent algorithms are upper-bounded by the optimal algorithm for the latter distribution even when the true distribution is the former. Thus, the ratio of the expected performances of the Bayesian optimal algorithms for these two decompositions is a lower bound on the prior independent approximation ratio. The techniques of the paper connect prior independent algorithm design, Yao's Minimax Principle, and information design. We apply this framework to give new lower bounds on several canonical prior independent mechanism design problems.

==> bib_work.tex <==

%  this bib contains references "to be moved," and gives the reason that they were added here

% from HJL: A mechanism's revenue can be easily and geometrically understood via the marginal revenue approach of \citet{mye-81} and \citet{BR-89}.
@ARTICLE{BR-89,
 author={J. Bulow and J. Roberts},
 title={The Simple Economics of Optimal Auctions},
 JOURNAL={The Journal of Political Economy},
 VOLUME=97,
 YEAR={1989},
 PAGES={1060-90},
 ISSUE=5
}

==> fig/triangle.tex <==
\begin{tikzpicture}[scale = 0.7]

\draw (-0.2,0) -- (10, 0);
\draw (0, -0.2) -- (0, 5.5);


\draw (0, 0) -- (3, 5);
\draw (3, 5) -- (9, 0);

\draw [dotted] (0, 5) -- (3, 5);
\draw [dotted] (3, 0) -- (3, 5);



\draw (0, -0.5) node {$0$};
\draw (-0.5, 5) node {$1$};

\draw (9, -0.5) node {$1$};
\draw (3, -0.5) node {$\monoq$};


\end{tikzpicture}



==> p_extra.tex <==

\newcommand{\cal}{\mathcal}
